Sli2Vol: Annotate a 3D Volume from a Single Slice with Self-Supervised Learning

The objective of this work is to segment any arbitrary structures of interest (SOI) in 3D volumes by only annotating a single slice, (i.e. semi-automatic 3D segmentation). We show that high accuracy can be achieved by simply propagating the 2D slice segmentation with an affinity matrix between consecutive slices, which can be learnt in a self-supervised manner, namely slice reconstruction. Specifically, we compare the proposed framework, termed as Sli2Vol, with supervised approaches and two other unsupervised/ self-supervised slice registration approaches, on 8 public datasets (both CT and MRI scans), spanning 9 different SOIs. Without any parameter-tuning, the same model achieves superior performance with Dice scores (0-100 scale) of over 80 for most of the benchmarks, including the ones that are unseen during training. Our results show generalizability of the proposed approach across data from different machines and with different SOIs: a major use case of semi-automatic segmentation methods where fully supervised approaches would normally struggle. The source code will be made publicly available at https://github.com/pakheiyeung/Sli2Vol.

==> sec/dataset.tex <==
\section{Dataset}
\label{sec:data}
% ====================
% Abdominal and Chest CT
% ====================
\subsection{Abdominal and Chest CT}

\subsubsection{Training Dataset}
Three public datasets from The Cancer Imaging Archive (TCIA)~\cite{clark2013cancer} were used for training.

\begin{enumerate}[(I)]
\item C4KC-KiTS~\cite{c4kc}: 
310 volumes acquired from 153 patients with kidney cancer who were treated by either partial or radical nephrectomy at the University of Minnesota Medical Center were used for training~\cite{heller2019kits19}.
The scans were collected at different referring institutions so different scanners and acquisition protocols were involved, resulting in heterogeneous image quality. 
The resolutions of the volumes are 512$\times$512 pixels with varying slice thickness.

\item CT-Lymph Nodes~\cite{lymphnodes}: 
86 CT volumes of the mediastinum and abdomen from different subjects were used for training. 
Different scanners and acquisition protocols were used for acquiring the volumes.
The resolutions of the volumes are 512$\times$512 pixels with varying slice thickness.


\item CT-Pancreas~\cite{pancreasct}: 
82 abdominal contrast enhanced 3D CT scans were acquired from 53 male and 27 female subjects, with ages range from 18 to 76 years (mean age of 46.8 $\pm$ 16.7). 
The resolutions of the volumes are 512$\times$512 pixels with varying slice thickness between 1.5 - 2.5 mm. 
The volumes were acquired from Philips and Siemens MDCT scanners (120 kVp tube voltage).

%The National Institutes of Health Clinical Center performed 82 abdominal contrast enhanced 3D CT scans (~70 seconds after intravenous contrast injection in portal-venous) from 53 male and 27 female subjects.  Seventeen of the subjects are healthy kidney donors scanned prior to nephrectomy.  The remaining 65 patients were selected by a radiologist from patients who neither had major abdominal pathologies nor pancreatic cancer lesions.  Subjects' ages range from 18 to 76 years with a mean age of 46.8  16.7. The CT scans have resolutions of 512x512 pixels with varying pixel sizes and slice thickness between 1.5 - 2.5 mm, acquired on Philips and Siemens MDCT scanners (120 kVp tube voltage).

\end{enumerate}

\subsubsection{Testing Dataset}
8 public datasets with 9 different ROIs were used for testing.

\begin{enumerate}[(I)]
\item Sliver07~\cite{van07}: 
20 CT volumes with liver annotation were used for testing.
The scans were acquired from a variety of CT scanners (i.e. different manufacturers, 4, 16 and 64 detector rows). 
The resolutions of the volumes are 512$\times$512 pixels with pixel spacing between 0.55 and 0.80 mm and inter-slice distance from 1 to 3 mm without overlapping between slices. 

\item CHAOS~\cite{CHAOSdata2019}: 
20 upper abdominal CT volumes, acquired from healthy subjects, with liver annotation were used for testing.
The scans were acquired from three different CT scanners (i.e. Philips SecuraCT with 16 detectors and a Philips Mx8000 CT with 64 detectors and Toshiba AquilionOne with 320 detectors).
The resolutions of the volumes are 512$\times$512 pixels with pixel spacing between 0.7-0.8 mm and inter-slice distance from 3 to 3.2 mm.

%The first database contains CT images of 40 different patients. These patients are potential liver donors, who have healthy (no tumors, lesions or any other diseases) liver. The CT images were acquired from upper abdomen area of the patients at portal venous phase after contrast agent injection. Portal venous phase is the phase obtained 70-80 sec after contrast agent injection or 50-60 sec after bolustracking. In this phase the liver parenchyma enhances maximally through bloodsupply by the portal vein. Portal veins are well enhanced and some enhancement of the hepatic veins is also seen on the portal venous phase. Therefore, this phase is widely used for the liver and vessel segmentation prior to surgery.
%
%Three different modalities, Philips SecuraCT with 16 detectors and a Philips Mx8000 CT with 64 detectors and Toshiba AquilionOne with 320 detectors (all equipped with the spiral CT option), are used. The patient orientation and alignment is the same for all data sets. Each data set consists of 16 bit DICOM images with a resolution of 512x512, x-y spacing between 0.7-0.8 mm and having 3 to 3.2 mm inter-slice distance (ISD) (i.e. smaller ISD is not being used for these acquisitions due to the routine clinical procedure). This corresponds to an average of 90 slices per data set (i.e. minimum 77, maximum 105 slices). In total, 1367 slices will be provided for training and 1408 slices will be used for tests. The challenges of the data set can be summarized as:

\item 3D-IRCADb-01~\cite{soler20103d}: 
20 CT volumes, acquired from 10 male and 10 femal subjects, with multiple annotated organs were used for testing.
The annotated ROIs we analyzed include heart, gallbladder, kidney, surrenalgland, liver, lung, pancreas and spleen.
The resolutions of the volumes are 512$\times$512 pixels with varying slice thickness.

\item 3D-IRCADb-02~\cite{soler20103d}: 
2 anonymized thoraco-abdominal enhanced CT volumes with multiple annotated organs were used for testing.
The first one was acquired during the arterial phase in inhaled position while the second scan was acquired during the portal phase in exhaled position.
The annotated ROIs we analyzed include heart, gallbladder, kidney, surrenalgland, liver, lung, pancreas and spleen.
The resolutions of the volumes are 512$\times$512 pixels with varying slice thickness.

\item Decathlon-Spleen~\cite{simpson2019large}: 
41 CT volumes with spleen annotation were used for testing.
The volumes were reconstructed with a standard convolutional kernel and with a reconstruction diameter range of 360–500 mm, and slice thickness between 2.5 - 5 mm.

\item Decathlon-Liver~\cite{simpson2019large, bilic2019liver}: 
131 volumes acquired at 6 different clinical sites, from patients with a variety of primary cancers who were either undergoing or finishing therapy, were used for testing.
Some of the volumes were corrupted with metal artifacts, which is commonly seen in real-world clinical scenarios. 
The resolutions of the volumes vary from 0.5 - 1.0 mm with varying slice thickness between 0.45 to 6.0 mm.

\item Decathlon-Pancreas~\cite{simpson2019large}: 
281 CT volumes with pancreas annotation were acquired from patients undergoing resection of pancreatic masses and used for testing.
The resolutions of the volumes are 512$\times$512 pixels with inter-slice distance of 2.5 mm. 


\end{enumerate}

% ====================
% Cardiac MRI
% ====================
\subsection{Cardiac MRI}

\subsubsection{Training Dataset (Kaggle)}
Data from the Kaggle Second National Data Science Bowl~\cite{kaggle} were used for training. 
The dataset contains 14370 video sequences acquired from 1140 patients and each sequence is composed of around thirty 2D cine images across the cardiac cycle.
For each patients, video sequences of different views, including short axis stack, 2-chamber and 4-chamber views, are included. 
Different scanners and acquisition protocols were used for acquiring the images.

\subsubsection{Testing Dataset (Decathlon-Heart)}
20 MRI volumes spanning the whole heart acquired during a single cardiac phase with left atrium annotation were used for testing~\cite{simpson2019large}.
The scans were acquired from a 1.5T Achieva scanner (Philips Healthcare, Best, The Netherlands) with resolution 1.25$\times$1.25$\times$2.7 $mm^3$.




==> sec/related.tex <==
\section{Related Works}
\vspace{-5pt}
\par{\noindent \textbf{Semi-automatic Segmentation}} 
for 3D medical volumes are normally approached using level set method.
Generally, one or more seeds of the SOI are provided by the user during inference time. 
In the literature, 
excellent performance have been reported in~\cite{zheng2018unified, foruzan2016improved, li2013likelihood, dawant2007semi}.
However, these approaches heavily rely on parameter-tuning for different modalities or SOIs, 
and the running time can sometimes be up to tens of minutes for a large volume.
These deficiencies have clearly limited their use in real-world applications, 
and indeed, only 1-2 modalities or SOIs were benchmarked in each of the previous studies.
To this end, 
this paper focuses on the generalization capability and fast inference, 
where the goal is to train a model that is applicable to different domains~(\eg~across different machines and SOIs) 
\emph{without} any parameter-tuning during inference, 
in addition, 
it requires less than 30 seconds to process a large volume, 
which is orders of magnitude faster than conventional approaches. \\[-5pt]

\par{\noindent \textbf{Few-shot Segmentation}} 
refers to the problem where only limited annotation is provided to train segmentation models.
In general, it has been approached by following a pretrain and fine-tune paradigm, 
in which models trained with abundant data are fine-tuned with the given few annotations for the downstream task.
In~\cite{caelles2017one}, 
an one-shot video segmentation framework was proposed by fine-tuning image classification CNNs
for video segmentation, given the mask of the first video frame.
%Despite the state-of-the-art performance achieved, 
%model pretrained on large annotated datasets ($i.e.$ ImageNet and DAVIS) is required,
%which is unavailable in the medical imaging field.
As for medical image analysis, 
\cite{roy2020squeeze} proposed to use a two-stream CNNs,
one stream processes the annotated image slice and generates task-specific representation,
which is further used for re-weighting the parameters in the other `segmenter' stream.
During inference, a few slices of a volume are annotated, 
\ie~few-shot, to steer the segmentation of a similar \emph{query} volume.
In both studies, a fair amount of annotations is required for training data,
and test-time fine-tuning is necessary.
Our study performs the similar \emph{one-shot segmentation} task without such prerequisites.


%\par{\noindent \textbf{Few-shot Segmentation}} 
%refers to the problem where  only limited annotaiton is provided to segmentation models.
%In general, this problem has been approached by fine-tuning a pretrained-model (\ie~trained for different tasks) with the given few annotations.
%In~\cite{roy2020squeeze} proposes a few-shot segmentation framework that utilizes a few annotated slices of a volume as support training data to guide the segmentation of other slices of the volume.
%\weidi{this is not clear, how did they train the model ? support training data means ? they do nearest neighbor way ? }
%Another study~\cite{zhao2019data} tries to tackle MRI brain segmentation by learning the transformation from an annotated atlas to scans in an unlabelled dataset, 
%which can then be used to synthesize new volumes and annotations to train models in a fully-supervised manner.
%Unlike these work, we focus on the paradigm of mask propagation.
%\weidi{this few shot segmentation is not clear to me, how the previous papers define the problem ? the given annotation is for a few volume ? or each volume few slices ? these are different problem setting, need to be clear if we are doing something different from theirs.}

 
%but only one or two modalities or ROIs were tested in each study.
%The performance of these approaches depends heavily on fine-tuning of different parameters and different regularizations based on prior knowledge, for example shape, position and intensity distribution about the modalities and ROIs, which make generalization much harder.
%On the other hand, our proposed framework targets on generalizing to different modalities and one single trained model can be used for different ROIs without any fine-tuning during inference. 
%This may be more suitable for the need in daily application.
%In addition, the running time needed for each volume using approaches based on level set method normally ranges from a few to up to tens of minutes, depending on the size of the volume.
%This impedes interactive segmentation.
%Our proposed framework, on the other hand, requires less than 30 seconds for a large volume, which is orders of magnitude faster. \weidi{this is too long, shorten it.}

%\weidi{we are simply inspired by the tracking idea, but this is too large jump for reviewers, if you want to mention it,
%this has to be merged into the semi-automatic segmentation paragraph, and shorten it into one or two sentences.}
%Semi-automatic segmentation (or dense tracking or semi-supervised video segmentation) 
%is a popular research area in the field of natural image processing.
%The problem is normally formulated as tracking of a ROI densely in a video, given the mask in the first frame of the video.
%In recent years, unsupervised or self-supervised approaches based on 
%optical flow~\cite{ren2017unsupervised, Meister:2018:UUL, jonschkowski2020matters}
%or dense correspondence~\cite{Lai19, lai2020mast} 
%were proposed.
%Basically, these studies rely on training a model on pair of adjacent frames by reconstructing the second frame by the first frame based on the optical flow field or correspondence mapping predicted by the model.
%The reconstructed and original second frame can then be used to supervise the learning through minimizing their difference.
%Our work relies on similar principle by predicting a flow field from one slice to another slice sampled from a 3D volume.
%We further investigate on a verification module to correct the propagated mask during inference, which is seldomly studied due to the difference of nature between 3D medical volumes and natural video sequences.
%
%
%\weidi{One more related works.}
